Analysis and Prevention of MCAS-Induced Crashes

Semi-autonomous (SA) systems face the challenge of determining which source to prioritize for control, whether it's from the human operator or the autonomous controller, especially when they conflict with each other. While one may design an SA system to default to accepting control from one or the other, such design choices can have catastrophic consequences in safety-critical settings. For instance, the sensors an autonomous controller relies upon may provide incorrect information about the environment due to tampering or natural fault. On the other hand, the human operator may also provide erroneous input. To better understand the consequences and resolution of this safety-critical design choice, we investigate a specific application of an SA system that failed due to a static assignment of control authority: the well-publicized Boeing 737-MAX Maneuvering Characteristics Augmentation System (MCAS) that caused the crashes of Lion Air Flight 610 and Ethiopian Airlines Flight 302. First, using a representative simulation, we analyze and demonstrate the ease by which the original MCAS design could fail. Our analysis reveals the most robust public analysis of aircraft recoverability under MCAS faults, offering bounds for those scenarios beyond the original crashes. We also analyze Boeing's updated MCAS and show how it falls short of its intended goals and continues to rely upon on a fault-prone static assignment of control priority. Using these insights, we present Semi-Autonomous MCAS (SA-MCAS), a new MCAS that both meets the intended goals of MCAS and avoids the failure cases that plague both MCAS designs. We demonstrate SA-MCAS's ability to make safer and timely control decisions of the aircraft, even when the human and autonomous operators provide conflicting control inputs.

==> 000-Results/_fic-mcas-new-old-safe-state.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.8\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{000-Results/RTAS-24-SAFE-STATE-OLD.pdf}
        \caption{\small \mcasold.}
        \label{fig:mcas_old_safe_state}
    \end{subfigure}
    \begin{subfigure}[b]{0.8\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{000-Results/RTAS-24-SAFE-STATE-NEW.pdf}
        \caption{\small \mcasnew}
        \label{fig:mcas_new_safe_state}
    \end{subfigure}
    \caption{\small 
    \color{red} Evaluation of timing analysis for aircraft recovery given varying recovery times and exerted rotational effort on the HS.
    }
    \label{fig:mcas_new_old_safe_state}
    \vspace{-0.2in}
\end{figure}

==> 000-Results/_fig-mcas-new-all.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\columnwidth]{000-Results/RTSS-23-MCAS-NEW-ALL-COLOR-BIG-2.pdf}
    \caption{\small Summary of \mcasnew{} simulation. Success rate: 266/295 = 90.17\%}
    \label{fig:mcas_new_all}
    \vspace{-0.2in}
\end{figure}

==> 000-Results/_fig-mcas-new-old-and-old-adapt.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.8\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{000-Results/RTSS-23-MCAS-OLD-ALL-COLOR-BIG-FINAL.pdf}
        \caption{\small \mcasold{} (271/795 = 34.09\%)}
        \label{fig:mcas_old_all}
    \end{subfigure}
    % \begin{subfigure}[b]{0.3\textwidth}
    %     \centering
    %     \includegraphics[width=\columnwidth]{000-Results/RTSS-23-MCAS-OLD-ADAPT-ALL-COLOR-BIG-FINAL.pdf}
    %     \caption{\small \mcasoldadj{} (307/780 = 39.36\%)} %15 dropped from delta duration bc the sim would crash for 66-80
    %     \label{fig:mcas_old_adapt_all}
    % \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.8\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{000-Results/RTSS-23-MCAS-NEW-ALL-COLOR-BIG-FINAL.pdf}
        \caption{\small \mcasnew{} (764/795  = 96.10\%)}
        \label{fig:mcas_new_all}
    \end{subfigure}
    \caption{\small 
    Summaries of stress test simulation trajectories. 
    Each is labeled with the MCAS type and the 
    corresponding success rate in parentheses. Some 
    colors in the legend are non-visible since they 
    overlap with the trajectories of other colors.
    }
    \label{fig:mcas_new_old_adapt}
    \vspace{-0.2in}
\end{figure}

==> 000-Results/_fig-mcas-old-adapt-all.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\columnwidth]{000-Results/RTSS-23-MCAS-OLD-ADAPT-ALL-COLOR-BIG-2.pdf}
    \caption{\small Summary of \mcasoldadj{} simulation. Success rate: 230/295 = 77.97\%}
    \label{fig:mcas_old_adapt_all}
    \vspace{-0.2in}
\end{figure}

==> 000-Results/_fig-mcas-old-all.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\columnwidth]{000-Results/RTSS-23-MCAS-OLD-ALL-COLOR-BIG-2.pdf}
    \caption{\small Summary of \mcasold{} simulation. Success rate: 150/295 = 50.85\%}
    \label{fig:mcas_old_all}
    \vspace{-0.2in}
\end{figure}

==> 000-Results/_fig-sa-mcas-adapt-all.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\columnwidth]{000-Results/RTSS-23-SA-MCAS-ADAPT-ALL-COLOR-BIG-2.pdf}
    \caption{\small Summary of \nameadj{} simulation. Success rate: 272/295 = 92.20\%}
    %% ==$>$ All are when pilot stalls and delays $>$6s
    \label{fig:sa_mcas_adapt_all}
    \vspace{-0.2in}
\end{figure}

==> 000-Results/_fig-sa-mcas-all.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\columnwidth]{000-Results/RTSS-23-SA-MCAS-ALL-COLOR-BIG-2.pdf}
    \caption{\small Summary of \name{} simulation. Success rate: 272/295 = 92.20\%}
    % ==$>$ All are when pilot stalls and delays $>$6s
    \label{fig:sa_mcas_all}
    \vspace{-0.2in}
\end{figure}

==> 000-Results/_fig-sa-mcas-and-sa-mcas-adapt.tex <==
\begin{figure*}
    % \centering
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\columnwidth]{000-Results/RTSS-23-SA-MCAS-ALL-COLOR-BIG-FINAL.pdf}
        \caption{\small \name{} (770/795 = 96.86\%)}
        \label{fig:sa_mcas_all}
    \end{subfigure}
    % \hspace{5em}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\columnwidth]{000-Results/RTSS-23-SA-MCAS-ADAPT-ALL-COLOR-BIG-FINAL.pdf}
        \caption{\small \nameadj{} (770/795 = 96.86\%)}
        \label{fig:sa_mcas_adapt_all}
    \end{subfigure}
    \caption{\small
    Summaries of \name{} simulations. Each is labeled 
    with the MCAS type and the corresponding success 
    rate in parentheses. Some colors in the legend are 
    non-visible since they perfectly overlap with the 
    trajectories of other colors.
    }
    \label{fig:sa_mcas_and_sa_mcas_adapt}
    \vspace{-0.1in}
\end{figure*}

==> 300-Background/_fig-hs_aoa.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{300-Background/aoa-hs.pdf}
    \caption{\small Relevant information for the pitch of an aircraft.
    The Angle of Attack (AoA) is defined as the difference between the chord line and flight path of the aircraft. The elevator and horizontal stabilizer are the actuators responsible for pitch control. Image in circle from~\cite{crowley:flickr}.}
    \label{fig:hs_aoa}
    \vspace{-0.2in}
\end{figure}

==> 300-Background/background-prior-work.tex <==
Insofar, it is clear that a well-designed and safety-aware 
SA system should not default control to either the pilot 
or autonomous entity in the face of conflicting control.
We survey the prior work that examines dynamic control
authority.

{\color{red} TBD}

% {\color{red}
% Whether dealing with one autonomous driver
% \cite{shia:14:tits,gray:13:iv,weiskircher:tcst:17,rajamani:02:tvt,altche:17:tits,vasudevan:12:acc}
% or both an autonomous and human driver
% \cite{huang:19:thms,nguyen:21:sensors,anderson:12:iv,wray:16:aamas,wyk:20:tret},
% failing to investigate the correctness of control
% decisions and properly granting them permission
% creates this point-of-failure.
% CCC: All related to cars. Relevant here?
% }

==> 310-Threat_Model/_fig-threatmodel.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.9\columnwidth]{310-Threat_Model/threat_model.pdf}
    \caption{\small An overview of the threat model for SA control
        of the pitch of an aircraft.}
    \label{fig:threat}
    \vspace{-0.2in}
\end{figure}

==> 500-Challenges/_fig-sa_mcas.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.88\columnwidth]{500-Challenges/sa-mcas.pdf}
    \caption{\small The \name{} control-loop. \name{} and the pilot control input
    pass through the \name{} Arbiter to dynamically control the SA system.}
    \label{fig:sa_mcas}
    \vspace{-0.2in}
\end{figure}

==> 600-Implementation/_fig-model_architecture.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{600-Implementation/model-architecture.pdf}
    \caption{\small The model architecture for the \name{} arbiter.
    The architecture is an ensemble learning model that uses the stacking
    approach. The $n$ classifiers combine their predictions into a single
    meta-classifier that performs a final prediction. This final prediction
    determines arbitration for input to the pitch controller.}
    \label{fig:model_architecture}
    \vspace{-0.2in}
\end{figure}

==> 600-Implementation/_tbl-correlations.tex <==
\begin{table}
    \centering
    {\footnotesize
    \begin{tabular}{|| c | c | c ||} 
        \hline
        \textbf{Sensor \#1} & \textbf{Sensor \#2} & \textbf{Corr. Val.} \\ [0.5ex] 
        \hline\hline
        Altitude & Temperature & -0.85 \\
        Altitude & Air pressure & -0.99 \\
        $\Delta$Altitude & Pitch & -0.98 \\
        $\Delta$Altitude & $x$ acceleration & 0.81 \\
        % $\Delta$Altitude & Engine \% & 0.75 \\
        % $\Delta$Altitude & Throttle & 0.73 \\
        Pitch & $x$ acceleration & 0.86 \\
        % Pitch & Engine \% & 0.77 \\
        % Pitch & Throttle \% & 0.76 \\
        Roll & $\Delta$Heading & 0.95 \\
        $\Delta$Roll & Yaw acceleration & 0.94 \\
        $x$ acceleration & Engine \% & 0.87 \\
        $x$ acceleration & Throttle & 0.86 \\
        % $y$ acceleration & $z$ acceleration & -0.77 \\
        % $y$ acceleration & Roll acceleration & 0.70 \\
        $z$ acceleration & Roll acceleration & -0.80 \\
        Engine \% & Throttle & 0.95 \\
        Temperature & Air pressure & 0.91 \\
        \hline
    \end{tabular}
    }
    \caption{\small Sensor pairs with an absolute correlation
    $\geq$0.8. A $\Delta$ signifies a rate of change of
    the stated sensor.}
    \label{tbl:correlations}
    \vspace{-0.2in}
\end{table}

==> 600-Implementation/_tbl-dataset.tex <==
\begin{table*}
    \centering
    {\footnotesize
    \begin{tabular}{|| c | c | c | c ||} 
        \hline
        \rowcolor{black!10}
        \bf Maneuver & \bf Parameter(s) Adjusted & \bf \# Collected & \bf Mission Success Metric(s) \\ [0.5ex] 
        \hline\hline
        % Level & N/A & & Maintain level altitude ($\pm10$ ft) \\
        % \hline
        Accelerate & \makecell*{Initial airspeed (kts) \\Final airspeed (kts)} & 121 & Maintain level altitude ($\pm10$ ft) \\
        \hline
        Climb & \makecell*{Initial altitude (ft) \\Final altitude (ft)} & 100 & \makecell*{Maintain acceptable g-force ($0<$ and $<3g_0$)\\Maintain level altitude along expected route ($\pm10$ ft)} \\
        \hline
        Descend & \makecell*{Initial altitude (ft) \\Final altitude (ft)} & 100 & \makecell*{Maintain acceptable g-force ($0<$ and $<3g_0$)\\Maintain level altitude along expected route ($\pm10$ ft)} \\
        \hline
        Level-Turn & \makecell*{Initial heading ($^\circ$) \\Turn amount ($^\circ$)} & 101 & Maintain level altitude ($\pm10$ ft) \\
        \hline
        Climb-Turn & \makecell*{Turn amount ($^\circ$) \\Climb amount (ft)} & 121 & \makecell*{Maintain acceptable g-force ($0<$ and $<3g_0$)\\Maintain level altitude along expected route ($\pm10$ ft)} \\
        \hline
        Descend-Turn & \makecell*{Turn amount ($^\circ$) \\Climb amount (ft)} & 121 & \makecell*{Maintain acceptable g-force ($0<$ and $<3g_0$)\\Maintain level altitude along expected route ($\pm10$ ft)} \\
        \hline
        Holding Pattern & \makecell*{Initial heading ($^\circ$)\\Inbound/outbound leg time (s)} & 169 & Maintain level altitude ($\pm10$ ft) \\
        \hline
        Takeoff & \makecell*{Initial climb airspeed (kt)\\Climb phase transition altitude (ft)\\Final climb airspeed (kt)\\Final altitude (ft)} & 225 & \makecell*{Maintain an altitude $>0$\\Continue to increase in altitude} \\ 
        \hline
        Landing & \makecell*{Initial altitude (ft)\\Vertical descent rate (ft/s)\\Approach airspeed (kt)} & 100 & \makecell*{Reaches $<50$ ft with safe landing conditions\\(pitch $<4^\circ$; airspeed $<$ 120 kt)} \\
        \hline
    \end{tabular}
    }
    \caption{\small Summary of the dataset used in our evaluation.}
    \label{tbl:dataset}
    \vspace{-0.2in}
\end{table*}

==> 600-Implementation/_tbl-meta_classifier.tex <==
\begin{table}
    \centering
    % {\footnotesize
    % \begin{tabular}{|| c | c | c | c ||} 
    %     \hline
    %     Maneuver & Duration & Performed in Crash & Ref. \\ [0.5ex] 
    %     \hline\hline
    %     Level &  & $\bullet$ &  \\
    %     \hline
    % \end{tabular}
    % }
    \caption{\small Proposed meta-classifier models. \hl{WIP}}
    \label{tbl:meta_classifier}
    \vspace{-0.2in}
    %TODO: Thomas is putting together the documents for me
    % to enter into this table.
\end{table}

==> 600-Implementation/impl-02threats-mcasoldadapt.tex <==
% \input{000-Results/_fig-mcas-old-adapt-all}

\subsubsection{Sudden \& Delta Sensor Errors.}
Compared to \mcasold, \mcasoldadj{} provides
minor benefits, primarily related to timing.
An additional benefit is that the pilot can
sustain a slightly longer error.

\subsubsection{Gradual Sensor Errors.}
For the gradual errors, \mcasoldadj{} is
clearly the superior option. For the gradual
linear error, all cases were prevented from
impacting the ability to recover the flight.
Similar to \mcasold, this translated to the
portion of the quadratic gradual error that
represents the linear case. Outside of this,
the quadratic gradual error is unrecoverable.

\subsubsection{Pilot Stalling.}
Compared to \mcasold, the addition of
an adaptive cooldown in \mcasoldadj{} provides
no additional benefits to the cases where
the pilot stalls.

\subsubsection{Deadline \& Timing Analysis.}
Due to the adaptive cooldown feature of \mcasoldadj,
if the pilot reacts quicker than 4s, then they can
avoid a crash.

==> 600-Implementation/impl-03dataset.tex <==

To the best of our knowledge, there is no dataset robust enough 
for the purpose of our evaluation. Specifically, we require
a dataset that not only includes flight sensor data for
all of the standard flight maneuvers in \autoref{tbl:sim},
but also maneuvers that experience dangerous control.
While datasets such as OpenSky Network~\cite{schafer:14:ipsn} 
are available, they primarily use broadcast data that does 
not include crucial sensor data such as AoA. 
Thus, we need to create our own dataset.

%%
% The following is pretty useless here. Maybe useful later, so comment out.
%%%
% Because obtaining data from such dangerous flight conditions
% is unrealistic to obtain from a real aircraft, we turn
% to the use of a flight simulation tool. While we considered
% using a manual flight simulation tools such as FlightGear
% or Microsoft Flight Simulator in order to acquire data, our
% additional requirement of being able to replicate flight
% maneuvers necessitates an automatic simulation toolkit.
% One motivation for developing our own simulation toolkit
% is to meet this requirement, as JSBSim---the leading
% open-source flight dynamics simulator---can
% perform automatic simulations. Our extension to JSBSim
% was created in a way that would make use of this property
% of JSBSim, lending us the power to quickly generate a dataset.

% The dataset our toolkit produced is summarized in
% \autoref{tbl:dataset}.
Because MCAS is activated
during stall conditions, which are most likely
to occur during takeoff and landing, we focus much of our
attention on takeoff and landing maneuvers. We generated
takeoff maneuvers where the aircraft first ascends rapidly
during initial climb, then climbs more gradually after reaching a 
specified altitude. The aircraft continues to climb until it
arrives at a final cruising altitude, where it remains at level
flight. As for landing maneuvers, the aircraft starts at an
initial altitude and begins descending at a consistent
vertical speed. The aircraft reduces its speed to a target speed,
and maintains steady descent. Actual touchdown of the aircraft
is unnecessary since MCAS plays no role at this point, so
simulations are terminated upon reaching a very low altitude.
These takeoff and landing procedures are performed many times,
with several key parameters modified. 

In total, we simulated and collected data from 1158 flights,
totaling 133 simulated flight hours.

==> 600-Implementation/impl-03model.tex <==
A goal of \name{} is to make it
lightweight and efficient. Since we are deploying MCAS
on aircraft computing systems, we have to rely on
embedded compute resources that are not necessarily equipped
for more advanced statistical or machine learning models.
Since much prior work within this domain makes use of
correlation of sensor 
pairs~\cite{ganesan:17:wcx,he:20:dac,akowuah:21:rtas},
we opt to use a series of trained linear regression models, 
each representing a correlated sensor pair. 
Then, the estimated value from each regression
model is compared against the actual measured value. For each
comparison, if the difference between the two values is within 
a trained $\epsilon$, then we deem the sensor measurement to 
accurately measure the environment. Otherwise, the pair is
flagged for additional inspection. For the regression
estimates that do not match the measured value, we use several
correlated sensor pairs to pin down exactly which sensor of
the flagged pair is causing the inaccurate estimate.

\name{} does not have an adaptive detection
threshold $\epsilon_{adap}$,
which is traditionally used to counter sensor drift. Such scenarios
are considered in our error model through the gradual
injections. We are able to counter the accumulation
of measurement noise or small incremental signal spoofing
since MCAS will provide only one HS down command per
sensed stall event. Therefore, an error cannot trigger
a spree of HS down commands.

%%%% remove below since we are not working with an adversary
% Moreover, if the error
% attempts to use a stealthy noise-accumulation attack to
% remain just below the detection threshold, they still will be
% unable to trigger MCAS. This is because they also need to
% make the AoA sensors exceed the stall event detection boundary,
% which is 18$^\circ$. In order to achieve such a condition,
% the plane would need to be approaching a stall, meaning the 
% MCAS should fire a HS down command regardless of the attack.

To determine the correlated sensor pairs and train the linear
regression model, we use the dataset described in
\autoref{sec:prevention:dataset}.
During the training, we exclude the
data with sensor injections and dangerous pilot control that
we generated in \autoref{sec:threats}. This is because
the goal for the regression models is to understand normal
control input for correlated sensor pairs in order to later
infer when a particular control decision is normal. Of the
data in the dataset, we split 30\% for training
and 70\% for testing, where we split randomly between each 
maneuver type in order to have equal representation.

% \input{600-Implementation/_tbl-meta_classifier}

% \subsubsection{Closed-Form Data Relationships}
% \hl{WIP-NTC}

%\subsubsection
\noindent{\bf Correlated Sensor Pairs.}
We determine correlated pairs of sensed data across
each flight maneuver as well as all maneuvers as a whole.
Our findings for all maneuvers are summarized in 
\autoref{tbl:correlations}. We automatically drop pairs of 
sensors that have an absolute correlation $\leq$0.8. We
additionally use a relationship between the AoA and pitch
due to their values being closely coupled with one another.

\input{600-Implementation/_tbl-correlations}


==> 700-Results/_alg-recovery.tex <==
\begin{algorithm}[t]
    \KwData{The erroneous sensor data at the start of the recovery $\overline{{x}}_s(t_i)$, the time series of real sensor data $\boldsymbol{x}_s$, and the end of the injection $t_n$.}
    % \KwResult{$p$, the predicted position of the VRU.}
    $x_{diff} \gets |\overline{{x}}_s(t_i) - \boldsymbol{x}_s(t_i)|$\;
    $x_{curr} \gets \overline{{x}}_s(t_i)$\;
    \For{$t \in [t_i, t_n]$}{
        \eIf{$|x_{curr} - \boldsymbol{x}_s(t)| > 0.1*x_{diff}$}{
            \eIf{$\neg(\boldsymbol{x}_s(t) > x_{curr} \oplus x_{curr} > 0)$}{
                $x_{curr} \gets awgn(x_{curr} + 0.05*x_{curr})$\;
            }{
                $x_{curr} \gets awgn(x_{curr} - 0.05*x_{curr})$\;
            }
            $\overline{{x}}_s(t) \gets x_{curr}$\;
        }{
            $\overline{{x}}_s(t) \gets Kalman(\overline{{x}}_s(t-1))$\;
        }
    }
    \caption{\small Gradual Injection Recovery}
    \label{alg:recovery}
\end{algorithm}

==> 700-Results/_fig-sim.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[b]{\columnwidth}
        \centering
        \lstset{language=xml}
        \lstinputlisting{700-Results/io.xml}
        \lstset{language=json}
        \lstinputlisting{700-Results/anomaly.json}
        \caption{\footnotesize Code snippets for input/output 
        initialization and error injection.}
        \label{fig:sim:param}
    \end{subfigure}
    
    \begin{subfigure}[b]{\columnwidth}
        \centering
        \lstset{language=Matlab}
        \lstinputlisting{700-Results/mcas.m}
        \caption{\footnotesize Code snippet of the pre-crash MCAS 
        implementation.}
        \label{fig:sim:mcas}
    \end{subfigure}
    
    \begin{subfigure}[b]{\columnwidth}
        \centering
        \lstset{language=Matlab}
        \lstinputlisting{700-Results/pilot.m}
        \caption{\footnotesize Code snippet of a pilot performing
        the start of an aircraft takeoff.}
        \label{fig:sim:pilot}
    \end{subfigure}
    \caption{\small Example code simulating the sudden error injection
    on the AoA sensor during the Lion Air Flight 610 takeoff.}
    \label{fig:sim}
    % \vspace{-0.2in}
\end{figure}

==> 700-Results/_fig-threat-eval-delta.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{700-Results/delta_parametric_injection_amount.pdf}
        \caption{\footnotesize {\tt Val}.}
        \label{fig:injection:delta:val}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{700-Results/delta_parametric_injection_duration.pdf}
        \caption{\footnotesize {\tt EndTime}.}
        \label{fig:injection:delta:end}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{700-Results/delta_parametric_reaction.pdf}
        \caption{\footnotesize Pilot reaction time.}
        \label{fig:injection:delta:reaction}
    \end{subfigure}
    \caption{\small Analysis of {\em delta injection} for the stated variable on the original MCAS in a Boeing 737-800 MAX.}
    \label{fig:threat:eval:delta}
    \vspace{-0.1in}
\end{figure*}

==> 700-Results/_fig-threat-eval-gradual-breakdown.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{700-Results/gradual_parametric_injection_quad_coef_0.pdf}
        \caption{\footnotesize {\tt Coef1=0}.}
        \label{fig:injection:gradual:coef_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{700-Results/gradual_parametric_injection_quad_coef_0.1_0.4.pdf}
        \caption{\footnotesize {\tt Coef1=0.1} to {\tt 0.4}.}
        \label{fig:injection:gradual:coef_0.1_0.4}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{700-Results/gradual_parametric_injection_quad_coef_0.5_1.pdf}
        \caption{\footnotesize {\tt Coef1=0.5} to {\tt 1}.}
        \label{fig:injection:gradual:coef_0.5_1}
    \end{subfigure}
    
    \caption{\small Breakdown of {\tt Coef1} of the quadratic {\em gradual injection}.}
    \label{fig:threat:eval:gradual_breakdown}
    \vspace{-0.1in}
\end{figure*}

==> 700-Results/_fig-threat-eval-gradual.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{700-Results/gradual_parametric_injection_lin_coef.pdf}
        \caption{\footnotesize Linear {\tt Coef1}.}
        \label{fig:injection:gradual:lin}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{700-Results/gradual_parametric_injection_quad_coef.pdf}
        \caption{\footnotesize Quadratic {\tt Coef1}, {\tt Coef2}.}
        \label{fig:injection:gradual:quad}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{700-Results/gradual_parametric_injection_log_coef.pdf}
        \caption{\footnotesize Logarithmic {\tt Coef1}.}
        \label{fig:injection:gradual:log}
    \end{subfigure}
    
    \caption{\small Analysis of {\em gradual injection} for the stated function's coefficient on the original MCAS in a Boeing 737-800 MAX.}
    \label{fig:threat:eval:gradual}
    \vspace{-0.1in}
\end{figure*}

==> 700-Results/_fig-threat-eval-stall-sa-mcas.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.66\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{700-Results/sa_mcas_stall_all_settings_success.pdf}
        \caption{\footnotesize Recovered flights.}
        \label{fig:threat:eval:stall_sa_mcas:success}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.66\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{700-Results/sa_mcas_stall_all_settings_fail.pdf}
        \caption{\footnotesize Crashed flights.}
        \label{fig:threat:eval:stall_sa_mcas:fail}
    \end{subfigure}
    
    \caption{\small Pilot stalling Boeing 737-800 MAX with the 
        \name. Variables are the same as \autoref{fig:threat:eval:stall}.
        68/180 = 37.78\% of flights are recovered from crash.}
    \label{fig:threat:eval:stall_sa_mcas}
    \vspace{-0.2in}
\end{figure}

==> 700-Results/_fig-threat-eval-stall.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.66\columnwidth]{700-Results/stall_all_settings.pdf}
    \caption{\small Pilot stalling Boeing 737-800 MAX with the 
        post-crash revised MCAS. Variables are the target 
        pitch, final climb airspeed, and pitch up start time.}
    \label{fig:threat:eval:stall}
    \vspace{-0.2in}
\end{figure}

==> 700-Results/_fig-threat-eval-sudden.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{700-Results/sudden_parametric_injection_amount.pdf}
        \caption{\footnotesize {\tt Val}.}
        \label{fig:injection:sudden:val}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{700-Results/sudden_parametric_injection_duration.pdf}
        \caption{\footnotesize {\tt EndTime}.}
        \label{fig:injection:sudden:end}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{700-Results/sudden_parametric_reaction.pdf}
        \caption{\footnotesize Pilot reaction time.}
        \label{fig:injection:sudden:reaction}
    \end{subfigure}
    \caption{\small Analysis of {\em sudden injection} for the stated variable on the original MCAS in a Boeing 737-800 MAX.}
    \label{fig:threat:eval:sudden}
    \vspace{-0.1in}
\end{figure*}

==> 700-Results/_tbl-sa-mcas-stall.tex <==
\begin{table}
    \centering
    {\footnotesize
    \begin{tabular}{|| c | c ||} 
        \hline
        \textbf{Pitch Up Time} & \textbf{\# Success / \# Total} \\ [0.5ex] 
        \hline\hline
        80 sec. & 0/36 \\
        100 sec. & 5/36 \\
        120 sec. & 14/36 \\
        140 sec. & 21/36 \\
        160 sec. & 28/36 \\
        \hline
    \end{tabular}
    }
    \caption{\small Successful flight recoveries broken down by
    the time the pilot dangerously pitches up into a stall.}
    \label{tbl:sa_mcas_stall}
    \vspace{-0.2in}
\end{table}

==> 700-Results/criteria-03prevention.tex <==
During the evaluation of the \name{} arbiter,
our metric of concern is primarily of overall flight
safety. In other words, after injecting erroneous
data or commanding the pilot to perform a dangerous
control input, we are most concerned with whether
\name{} intervenes to prevent the simulated flight
from crashing. As we show in our preliminary study in
\autoref{fig:prestudy}, the individual MCAS versions
are capable of preventing {\em separate} dangerous
control, but our evaluation seeks to prevent {\em both}.

Thus, an important aspect to our evaluation is
whether, ultimately, the aircraft safely {\em finishes}
its mission. Here, we define ``mission" to mean the
duration of any particular maneuver, but a more precise
definition would mean the journey of an airplane from
takeoff to landing. Since the latter definition is too
general, we use the former definition to provide
a more fine-grained assessment of each type of dangerous
control that we studied in \autoref{sec:threats}.
In doing so, we provide a rigorous argument for the success
of \name.
%necessary vv ?
To clarify what it means for a mission to
finish successfully, we provide metrics for distinguishing
success from failure for each maneuver, included in
\autoref{tbl:dataset}.


==> 700-Results/result-02threats.tex <==
% \input{700-Results/_fig-threat-eval-sudden}
% \input{700-Results/_fig-threat-eval-delta}

% \input{700-Results/_fig-threat-eval-gradual}
% \input{700-Results/_fig-threat-eval-gradual-breakdown}
% \input{700-Results/_fig-threat-eval-stall}

To conduct experiments on the different types of sensor threats,
we perform a parametric analysis. For a given injection type, we
keep all inputs to the injection format constant except one, which
is the value we target for each analysis.

\subsubsection{Sudden \& Delta Injections}
\label{sec:threats:result:sudden_delta}
For the {\em sudden} and {\em delta injections}, we conduct 
three experiments for each injection: (1) {\tt StartTime=100},
{\tt EndTime=130}, and {\tt Val} set from {\tt 0} to {\tt 30}; 
(2) {\tt StartTime=100}, {\tt Val=18}, and {\tt EndTime} set 
from {\tt 110} to {\tt 180}. In experiments (1) and (2), 
the pilot reacts after 10 secs; (3) {\tt StartTime=100},
{\tt EndTime=130}, and {\tt Val=18}, and the pilot's reaction
set from 3 to 30 secs. The pilot's reaction
is a normalized elevator input of -0.3, followed by
a normalized elevator input of -0.15 after 10 more secs.
In each of the three experiments, the
original MCAS is used, and the range of values for the variable
has an increment of 1. The results of these simulations for
the {\em sudden} and {\em delta} injections
are summarized in \autoref{fig:threat:eval:sudden} and 
\autoref{fig:threat:eval:delta}, respectively.

% \input{600-Implementation/_tbl-dataset}

The results for the {\em sudden injection} demonstrate
that even just exceeding the threshold of MCAS is
enough to trigger devastating impact. This is especially
apparent in \autoref{fig:injection:sudden:val}, which has
two distinct outcomes for the plane. The parametric
analyses of {\tt EndTime} and pilot reaction time
show that these variables impact the time-to-crash
(Figs.~\ref{fig:injection:sudden:end} and
\ref{fig:injection:sudden:reaction}).
%(\autoref{fig:injection:sudden:end} and
%\autoref{fig:injection:sudden:reaction}).

On the contrary, the results for the {\em delta injection}
show something more interesting, especially around the threshold
of MCAS activation. For instance, the analysis of {\tt Val} in
\autoref{fig:injection:delta:val} shows that there are some
recoverable scenarios of an MCAS misfire. In the case of
\autoref{fig:injection:delta:end}, a smaller {\tt EndTime}
can illicit either a recoverable flight or a slower descent
after an MCAS misfire. Finally, the pilot reaction time analysis
demonstrates an interesting pattern. As shown in 
\autoref{fig:injection:delta:reaction}, a later reaction can
allow the pilot to deflect the aircraft's decent into a
more graceful crash of the aircraft, whereas an earlier
reaction time may trigger an additional MCAS misfire and
quickly push the aircraft back into a quick decent.

\subsubsection{Gradual Injections}
\label{sec:threats:result:gradual}
For the {\em gradual injections}, we conduct three 
experiments, one for each of linear,
quadratic, and logarithmic functions. The controlled settings for
these experiments are {\tt StartTime=100}, {\tt EndTime=130}, 
and pilot reaction time of 10 secs for the linear and
quadratic simulations, and 22.5 secs for the logarithmic
simulations. {\tt Coef1} is the coefficient $a$ in each of
the three functions, and {\tt Coef2} is the coefficient
$b$ in the quadratic function. For the linear function,
we run simulations with {\tt Coef1=0} to {\tt 3} with a
step size of 0.1. For the quadratic function,
{\tt Coef1=0} to {\tt 1} and {\tt Coef2=0} to {\tt 3},
both with step sizes of 0.1.
And for the logarithmic function, {\tt Coef1=0} to
{\tt 200} with a step size of 1.
The pilot reaction works the same as in
\autoref{sec:threats:result:sudden_delta}, and the original
MCAS is used. The results of simulations are summarized 
in \autoref{fig:threat:eval:gradual}.

The gradual linear injections lead to three behaviors
that we notice (\autoref{fig:injection:gradual:lin}).
For the smaller values of {\tt Coef1}, the impact
is marginal or causes a very slow descent. As
{\tt Coef1>1}, we see the flight trajectory either
nosedive completely or nosedive into a last second
nose up before ultimately crashing. In the latter, it
appears that a more graceful landing is possible in
comparison to a nosedive.

In the case of the gradual logarithmic injection
(\autoref{fig:injection:gradual:log}),
the flight descends quicker for larger values of
{\tt Coef1}. In the case of smaller values, the descent
is more gradual, whereas larger values lead to a nose dive.

We break down the gradual quadratic injection simulations
based on {\tt Coef1}, shown in
\autoref{fig:threat:eval:gradual_breakdown}.
The breakdown shows that starting from {\tt Coef1=0}
(\autoref{fig:injection:gradual:coef_0}),
the gradual quadratic injection starts with the
behavior of the linear function
(\autoref{fig:injection:gradual:lin}). 
With progressive increases in {\tt Coef1}
(Figs.~\ref{fig:injection:gradual:coef_0.1_0.4} and
\ref{fig:injection:gradual:coef_0.5_1}),
the gradual quadratic injections converge toward
the behavior of a {\em sudden injection}
(\autoref{fig:injection:sudden:val}). An adversary
may benefit from a gradual quadratic injection
in order to achieve similar results as the
{\em sudden injection} without exhibiting an immediate
``sudden" jump to the target value.

\subsubsection{Pilot Dangerously Stalls Aircraft}
\label{sec:threats:result:stall}
In our final experiment on launching attacks on the
MCAS, we take the other side and simulate a pilot
attempting to dangerously stall out the aircraft equipped
with the post-crash MCAS. Our findings are summarized in 
\autoref{fig:threat:eval:stall}. In our simulations,
we control three parts of the pilot: the
pitch the pilot targets (from 25$^\circ$ to 50$^\circ$
in increments of 5), the final climb airspeed (from 225kt
to 275kt in increments of 10), and the pitch up start
time (from 80 sec. to 160 sec. in increments of 20).
As is clear in \autoref{fig:threat:eval:stall}, all 
simulations lead to a stall and ultimately crash
the aircraft through the subsequent nosedive.



==> 700-Results/timing-02threats.tex <==
{\color{blue} NOTES ABOUT WHAT TO ACCOMPLISH HERE

if MCAS wrongly activates, can the pilot return to the correct trim angle on time? in this case, we want to measure the return to around the full 2.5 degrees. (obviously, this is approximate. since there are some changes in airspeed due to the misfire, it will be slightly different in reality)

it should be obvious based on our input parameters if the pilot can finish recovering the aircraft before the next time it fires with our strict model

we can loosen the model and allow 1 or 2 "misses" from the pilot if there is a dynamic cooldown. perhaps in successive activations the pilot can recover the missing HS once they gain more cooldown time
}

==> 700-Results/timing-03prevention.tex <==
{\color{blue} NOTES ABOUT WHAT TO ACCOMPLISH HERE

if MCAS correctly engages, does it stop the pilot from doing the dangerous behavior and can the pilot appropriately recover the aircraft to steady flight on time? in this case, i think this is where your question comes in. i think we need to define the desired behavior. if we are in (A) take-off, then a higher pitch is necessary. returning to level flight is the incorrect course of action. if we are in (B) cruise altitude and something caused the plane to take a high pitch, then we probably do want to return to level flight. MCAS might overshoot and solve the problem (more likely in (A)) and it might undershoot and mostly solve the problem (more likely in (B)). in the case of (A), MCAS shouldnt engage again in theory, so we are less concerned about it firing again (because our assumption is that it isnt misfiring). in the case of (B), MCAS should engage again in theory, but only if the AoA hasnt be resolved, so perhaps the pilot should just enter stall recovery procedure and let MCAS handle the HS trimming automatically.

with loose model where we accept some misses for a dynamic cooldown, the balance is to see if the flight can recover more quickly in the above case of (B) i.e., an undershoot
}

==> 800-Discussion/disc-generalize.tex <==
{\color{red} Furthermore, the authors' approach focuses exclusively on improving the MCAS module used in Boeing aircrafts. They face three challenges: (1) design and evaluation of MCAS without a physical aircraft, (2) identification of control inputs and human pilots that threaten safety of the aircraft, and (3) evaluation of their own approach SA-MCAS in comparison to MCASold and the MCASnew module. All three challenges are limited to the use in Boeing as MCAS is used in these airplanes. Therefore, the chosen approach has limited applicability. In section "VIII. Generalization to other SA systems", the authors attempt to extend the applicability of the approach to other systems, but the section is too short to evaluate these statements.}

As we observed in \autoref{sec:intro}, static assignment
of control priority is a common approach in SA systems
and the consequences from this design decision are not
well documented. We conducted a case study of such 
decision through Boeing's two versions of MCAS, and 
then proposed a mechanism for providing dynamic arbitration 
of control between the manual and autonomous inputs.
With the lessons learned from the MCAS case study
and our proposed solution \name, we identify
a design schema that other flight control systems
and SA mobility systems may draw inspiration from.

{\bf Other Flight Control Systems.}
We focus on \autoref{alg:sa_mcas}.
While our development of the SADS arbiter was for use
by \name, there is no reason why other SA flight
control systems cannot use it.
Due to its flexibility to other sensors, the 
internal-external redundancy used in \name{} is 
easily extensible to provide sanity checks for 
flight control systems that require air data to 
trigger autonomous actions.
For this paper, we focused on the MCAS
case study due to its high impact, relevance, and
relative ease of obtaining publicly available information.
With similar easy-to-access information about how
an autonomous flight controller works, the SADS
arbiter may provide the necessary consistency
checks for the needed air data sensors.

{\bf Other SA Mobility Systems.}
For other mobility systems (e.g., cars, drones, or
tele-operated robotic vehicles), we may also 
extend or apply our framework. For instance, since
drones use similar air data as an aircraft, they may
directly make use of the SADS arbiter. However,
a land-vehicle may not use any of the same data,
but could use a different synthetic data system.
Moreover, these other mobility systems may have
access to information sharing networks, which may
be used as part of the consistency checking process.

==> 800-Discussion/disc-other-attacks.tex <==
% There are a few additional attacks that we
% would like to discuss further.

\paragraph{Instantaneous Injection of Incorrect Sensor Values}
The {\em instantaneous injection}
creates incorrect values at singular points
in a sensor's readings. These sort of injections
can either be {\em periodic} or {\em random}
in their behavior. While we do not evaluate
these here, \name{} assess each individual
sensor value. During our evaluation of the
three main injections in this paper, no singular
erroneous sensor value was missed by \name.

\paragraph{Pilot Provides Dangerous Nosedive Input}
Our evaluation of dangerous pilot input only
assesses a pilot attempting to stall the aircraft,
as this is the intended scenario for MCAS to activate.
In other words, MCAS is not equipped to detect
dangerous nose-down events and mitigate them.
Thus, our evaluation did not cover this
dangerous input. However, given that MCAS does
have the ability to control the HS of an aircraft,
it is possible that it {\em could} be given the
authority to control the HS for dangerous nose-down
events. In such a case, \name{} arbiter may be
used to counteract such an event and in order to
stop the aircraft from entering a nosedive.

\paragraph{Both Control Inputs are Erroneous}
We evaluated the cases where {\em either}
the pilot delivers dangerous manual control to the 
aircraft {\em or} the MCAS delivers unsafe 
autonomous control to the aircraft. 
What we did not evaluate is what happens when
{\em both} of these inputs are unsafe. 
A limitation to the current version of \name{} is 
that at least one of the control modes must be 
delivering safe control input. 
The problem of delivering safe control to an SA system 
where all actors/operators are attempting 
dangerous control has been studied in other, simpler 
domains. For instance, one can design an SA system
where we have full knowledge of its state-space. 
Then, we may only allow control of the SA 
system along state-space paths that guarantee its 
safety~\cite{musliner:95:ai}.
However, for more sophisticated systems such as aircraft,
providing a complete state-space is intractable due to the
exploding number of states one can generate. To alleviate
this issue, the prior work loosened the guarantees 
provided to the safety of the system in favor of a 
probabilistic approach to safe operation
\cite{atkins:99:agents,atkins:96:aaai,atkins:96:uai}.
Rather than generating the entire state-space, just a 
few important sections of the state-space are generated. 
During operation, the paths with the highest 
probability of safe operation are favored over those 
with lower probabilities of safe operation.

In our case, these solutions are complimentary to the
desired objective of \name. To extend them to our work,
we may define a set of safe states for the airplane to
wait (such as the holding pattern) while the \name{}
arbiter determines the correct course of action. Then, in
order to make the correct, safe control decision, we may
use prior work
on local view reconstruction to rebuild the
erroneous sensor data into the form that is most probably
correct~\cite{chen:22:thesis}. This option is the last
resort and undesirable
if we are capable of using a safe control decision that
is directly from either the pilot or MCAS.

==> util.tex <==
\newcommand{\newlyedited}[1]{{\color{red}#1}}
